Garbled EDA: Privacy Preserving Electronic Design Automation

The complexity of modern integrated circuits (ICs) necessitates collaboration between multiple distrusting parties, including thirdparty intellectual property (3PIP) vendors, design houses, CAD/EDA tool vendors, and foundries, which jeopardizes confidentiality and integrity of each party's IP. IP protection standards and the existing techniques proposed by researchers are ad hoc and vulnerable to numerous structural, functional, and/or side-channel attacks. Our framework, Garbled EDA, proposes an alternative direction through formulating the problem in a secure multi-party computation setting, where the privacy of IPs, CAD tools, and process design kits (PDKs) is maintained. As a proof-of-concept, Garbled EDA is evaluated in the context of simulation, where multiple IP description formats (Verilog, C, S) are supported. Our results demonstrate a reasonable logical-resource cost and negligible memory overhead. To further reduce the overhead, we present another efficient implementation methodology, feasible when the resource utilization is a bottleneck, but the communication between two parties is not restricted. Interestingly, this implementation is private and secure even in the presence of malicious adversaries attempting to, e.g., gain access to PDKs or in-house IPs of the CAD tool providers.

==> Introduction.tex <==
\section{Introduction}\label{sec:introduction}
%%\textit{The following subsections should be added here:\\
%%1. The information about general purpose and specific simulators should be provided here.
%%\textbf{The limitations of the specific simulators and overhead of general purpose simulators should be noted here. 
%%We can refer to the \cite{songhori2016garbledcpu} or \cite{songhori2019arm2gc}}\\
%%2. The input type of these simulators should be stated, which is the design (IP) in the Verilog format (or any HDL), and it should be mentioned that this input must remain secret to the customers.
%%3. A piece of abstract information about Secure Function Evaluation (SFE) should be provided.\\
%%4. State the possibility of using the Garbling technique to securely simulate an IP or a set of IPS via Garbled simulators. 
%%(The work of Yao and TinyGarble, should be mentioned here as proof of securely computation examples and GarbledCPU and ARM2GC should be stated as a practical implementation of Garbling technique.)\\
%%5. Our idea and contributions, which is the Garbling a simulator to protect the simulator target IP should be presented at the end of introduction section. 
%%(specifically, garbling a part of a simulator to simulate specific benchmarks).\\}

The globalization of semiconductor production has been on the rise owing to the lowered costs, innovation in creating smaller technologies and reduced time-to-market. This horizontal business model has also led to grave trust issues among various parties involved in the supply chain.

Reverse engineering, IP piracy, IC overbuilding, counterfeiting or repacking of old ICs have quickly become serious challenges for the IC supply chain. Once an attacker obtains the IP netlist, it can be illegally sold or used to design other ICs (IC piracy). Also, one can reuse the components extracted from competing products, thus revealing trade secrets. Also, any stage of the supply chain can be compromised by implanting malicious circuits by the attacker. This might be to sabotage the system or leak information. Various design for trust techniques were proposed to address this problem.

Let's look at the existing solutions and their limitations to combat the threats mentioned before.
%hardware Obfuscation
Hardware Obfuscation offers protections against reverse engineering of the hardware itself by either the manufacturer or end user, insertion of hardware Trojans by the manufacturer, and overproduction of the device. .This can be achieved by Logic Locking \cite{roy2010ending} which obfuscates the circuits by adding additional logic into the original design, if wrong key inputs are given it creates a wrong output.
%Logic Locking
Logic locking techniques can be used to protect the IP at almost all stages of the hardware development process. However, other than creating an overhead to the design, SAT based attacks, signal probability skew attacks, bypass attacks, and key sensitization attacks \cite{zamiri2019threats} against logic locking have rendered them useless as they were shown to successfully extract the key. 
%FORTIS
The intention of FORTIS is to protect against IP overuse by untrusted IP integrator and IC overproduction by untrusted Foundry. It implements a protocol between the fabricated chips and the SoC designers/IP owners to activate the chips for preventing IP overuse and IC overproduction. It uses logic encryption technique to obfuscate the netlist of an SoC/ 3PIP and can only be unlocked upon receiving a chip unlock key (CUK). FORTIS is computationally expensive as it uses different cryptographic algorithms like key generation, asymmetric encryption and signature generation. However, the major drawback of this protocol is that the CUK can still be obtained by the foundry, the whole point of privacy becomes moot \cite{guin2016fortis}.
%IEEE
Another approach of protecting hardware designs is to encrypt the HDL using cryptographic methods. This prevents the end users of these models from accessing the plaintext of the design and being able to maliciously influence it. The main method for this HDL encryption is defined in IEEE Standard P1735.
Encrypting the design enables vendors in preventing some basic attacks from end users namely counterfeiting the design or stealing secrets from within it. However, it does very little to protect against reverse engineering or any attacks at the manufacturing stage. Serious problems that lead to a side-channel leakage, and accordingly, to the disclosure of the keys were demonstrated. Some attacks allowed for full circuit definition recovery of the IP \cite{chhotaray2017standardizing}. Such attacks highlight the importance of EDA tools in protecting the confidentiality of IPs.

Encryption methods have become an integral part of frameworks conceived to take account of IP piracy. For this purpose, to remotely unlock ICs and IPs, an on-chip root-of-trust executing protocols between IPs and the IP-owner is required. As on-chip solutions could be expensive, the role of a trusted entity, which can unlock the IP, is played by electronic design automation (EDA) tools. In this regard, when using an EDA tool, the user may perform simulation, synthesis, and other processes on the IP; however, the tool should never disclose the IP in its plaintext format.

In this paper we will discuss how SFE schemes can be tailored to the needs of a secure compiler.  Our goal is to enable the user (IC designer) to obtain the technology mapped/optimized circuit without disclosing the information about the process design kit (PDK).The IP owner trusts the EDA tool vendor so that the raw IP is included in the source code of the tool. We use garbled circuits, a secure multi party computation protocol to achieve desired security involving two parties: the EDA tool and IC designer with PDK file as input.  We will show how using this approach no information on the inputs of the user (IC designer) is leaked to the EDA tool provider.

%EDA

State-of-the-art EDA tools provide powerful solutions for simulation, verification, and testing, and they are also well- tailored to optimize any design for power, performance, and area (PPA). However, these tools are neither tailored yet to account for, e.g., information leakage exploited by SCAs, nor do they offer to incorporate countermeasures in a way that maintains optimization and security guarantees.

It is understood that EDA tools cannot provide perfect security but it is an essential task to formulate and explore the practical bounds for security schemes when embedded in hardware. EDA tools should assist the designer with automated integration of security features and countermeasures but also needs to formulate the related limitations and remaining risks clearly, to enable effective risk management.\cite{knechtel2020towards}

Threats such as SCA, Fault-injection attacks, Piracy of design intellectual property (IP), counterfeiting of ICs and insertion of Hardware Trojans can occur during runtime, manufacturing or design phase. Some EDA measures have been proposed over the years to evaluate and mitigate such issues at design time.
There were fallacies in security of EDA as several EDA tools as well as design components and technology libraries are provided by potentially malicious third parties. This presents clearly one of the threats for secure composition of ICs. For example, Trojans could be introduced directly by adversarial designers, indirectly through untrustworthy third-party IP components, or even through “hacks” of EDA tools or the IT environment. 

==> Steffi.tex <==
%These were provided by Steffi in the 2nd section

%%1. Provide information about the concepts of PFE, the garbling method using Yaou, and oblivious transfer.\\
%%2. Briefly provide information about the last optimization of garbling.\\
%%3. The adversary type, which is honest-but-curious, should be stated. (similar papers stated that it is a norm that in this application the adversary model is honest-but-curious)


%\textbf{Security Model.} Classically, two main categories of adversaries have been considered. \textit{Semi-honest Adversary }is expected to execute the protocol correctly and not deviate from the protocol specification but may attempt to learn more from the information at hand. A \textit{Malicious Adversary} may arbitrarily deviate from the protocol execution and attempt to cheat. 

%\textbf{Oblivious Transfer.} \cite{naor2005computationally} Oblivious Transfer (OT) is a cryptographic protocol that runs between a Sender (\textit{S}) and a Receiver (\textit{R}). The receiver R obliviously selects one of the inputs provided by \textit{S}. Specifically, in a 1-out-of-\textit{n} \(OT_1^n\) protocol, the sender \textit{S} provides n-tuple \((x_1, ..., x_n )\) and the receiver \textit{R} has an index \textit{r} where \(1 \leq r \leq n\) and receives \(x_r\) among the sender’s messages without the sender learning the index \textit{r}, while the receiver only obtains one of the \textit{n} possible inputs. In our scenario we will use 1-out-of-2 for binary selection.
`

%\textbf{Yao's Garbled Circuit.} \cite{yao1986generate} In this MPC protocol two parties Alice (garbler) and Bob (evaluator) want to securely compute a function keeping their inputs private. The function \textit{f} is represented as a combinational Boolean circuit. For each gate, Alice symmetrically encrypts the respective output tokens with the four possible combinations of the input tokens, creating an encrypted truth table called the garbled table. Alice sends Bob the garbled tables and her own corresponding input value tokens. Using 1- out–of 2 OT, Bob receives the tokens corresponding to his input. Bob then decrypts the corresponding entry in the garbled table based on the received input tokens and gets the output. Finally, Alice will decrypt the output evaluated by Bob.

%EDA: Electronic design automation (EDA) for ICs has focused traditionally on power, performance, and area. However, given the rise of hardware-centric security threats, we believe that EDA must also adopt related notions like secure by design and secure composition of hardware. Encrypting the design enables vendors in preventing some basic attacks from end users namely counterfeiting the design or stealing secrets from within it. However, it does very little to protect against reverse engineering or any attacks at the manufacturing stage. Serious problems that lead to a side-channel leakage, and accordingly, to the disclosure of the keys were demonstrated. Some attacks allowed for full circuit definition recovery of the IP \cite{chhotaray2017standardizing}. Such attacks highlight the importance of EDA tools in protecting the confidentiality of IPs.


%Encryption methods have become an integral part of frameworks conceived to take account of IP piracy. For this purpose, to remotely unlock ICs and IPs, an on-chip root-of-trust executing protocols between IPs and the IP-owner is required. As on-chip solutions could be expensive, the role of a trusted entity, which can unlock the IP, is played by electronic design automation (EDA) tools. In this regard, when using an EDA tool, the user may perform simulation, synthesis, and other processes on the IP; however, the tool should never disclose the IP in its plaintext format.

%Threats such as SCA, Fault-injection attacks, Piracy of design intellectual property (IP), counterfeiting of ICs and insertion of Hardware Trojans can occur during runtime, manufacturing or design phase. Some EDA measures have been proposed over the years to evaluate and mitigate such issues at design time.
%Fallacies in security of EDA were noticed as several EDA tools as well as design components and technology libraries are provided by potentially malicious third parties. This presents clearly one of the threats for secure composition of ICs. For example, Trojans could be introduced directly by adversarial designers, indirectly through untrustworthy third-party IP components, or even through “hacks” of EDA tools or the IT environment. 

%State-of-the-art EDA tools provide powerful solutions for simulation, verification, and testing, and they are also well- tailored to optimize any design for power, performance, and area (PPA). However, these tools are neither tailored yet to account for, e.g., information leakage exploited by SCAs, nor do they offer to incorporate countermeasures in a way that maintains optimization and security guarantees. Our approach ensures protection against insertion of Hardware trojan and SCA.
%ASSURE is  an RTL locking framework against an untrusted foundry that has no access to an unlocked functional chip. ASSURE obfuscates the RTL by adding in opaque predicates such that the evaluation of the opaque predicates depends on the locking key; their values are known to the designer during obfuscation, but unknown to the untrusted foundry. ASSURE operates on the Verilog RTL description and is fully compatible with industrial EDA flows. ASSURE hides the essential semantics (constants, operations, and control-flow branches) in a way that's indiscernible and secure against attackers who don't have understanding of IP function priorly. It's been shown that the circuits can be unlocked only with the correct key of the obfuscated design. 


\cite{hu2020overview} \cite{koushanfar2012can}




